Informative Planning in the Presence of Outliers

Informative planning seeks a sequence of actions that guide the robot to collect the most informative data to build a large-scale environmental model or learn a dynamical system. Existing work in informative planning mainly focuses on proposing new planners and applying them to various robotic applications such as environmental monitoring, autonomous exploration, and system identification. The informative planners optimize an objective given by a probabilistic model, e.g., Gaussian process regression (GPR). In practice, the ubiquitous sensing outliers can easily affect the model, resulting in a misleading objective. A straightforward solution is to filter out the outliers in the sensing data stream using an off-the-shelf outlier detector. However, informative samples are also scarce by definition so they might be falsely filtered out. In this paper, we propose a method to enable the robot to re-visit the locations where outliers were sampled besides optimizing the informative planning objective. The robot can collect more samples in the vicinity of outliers and update the outlier detector to reduce the number of false alarms. We achieve this by designing a new objective for the Pareto Monte Carlo tree search (MCTS). We demonstrate that the proposed framework performs better than applying an outlier detector naively.

==> figures/figure.tex <==
\begin{figure}[tp]%
  \centering%
  \subfloat{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \fbox{\includegraphics[width=\linewidth]{example-image}}};%
      \end{tikzpicture}}}%
  \subfloat{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \fbox{\includegraphics[width=\linewidth]{example-image}}};%
      \end{tikzpicture}}}\\%
  \subfloat{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \fbox{\includegraphics[width=\linewidth]{example-image}}};%
      \end{tikzpicture}}}%
  \subfloat{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \fbox{\includegraphics[width=\linewidth]{example-image}}};%
      \end{tikzpicture}}}%
  \caption{Illustrations of the searching results of PUCT and UCT. In the occupancy map of (a), black and white colors represent occupied space and free space, respectively. In a reward map, darker color indicates higher reward value. The goal is to search a trajectory that maximizes the cumulative reward. The green tree shows the searching process which outputs the best trajectory colored in red and best action shown in blue. The first reward map tells the PUCT to search towards the upper right while the second reward map encourages going up. The reward map of the UCT is the same as the first reward map in (a). The PUCT balances the two rewards and gives different trajectory at the end.}%
  \label{fig:puct}%
\end{figure}


==> figures/figure1.tex <==
\begin{figure}[tp]%
  \centering%
  \subfloat[Chlorophyll level over time]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){\includegraphics[width=\linewidth,height=0.6\linewidth]{%
        ./images/figure1/chlorophyll.png}};%
      \end{tikzpicture}}}%
  \subfloat[Ground-truth model and data]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){\includegraphics[width=\linewidth,height=0.6\linewidth]{%
        ./images/figure1/data.png}};%
      \end{tikzpicture}}}\\%
  \subfloat[GPR without outliers]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){\includegraphics[width=\linewidth,height=0.6\linewidth]{%
        ./images/figure1/gpr_wo_outliers.png}};%
      \end{tikzpicture}}}%
  % \subfloat[Planning without outliers]{%
  %   \resizebox{0.5\linewidth}{!}{
  %     \begin{tikzpicture}%
  %       \node at(0.0,0.0){\includegraphics[width=\linewidth,height=0.6\linewidth]{%
  %       ./images/fig1_path_wo_outliers.png}};%
  %     \end{tikzpicture}}}\\%
  \subfloat[GPR with outliers]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){\includegraphics[width=\linewidth,height=0.6\linewidth]{%
        ./images/figure1/gpr_w_outliers.png}};%
      \end{tikzpicture}}}%
  % \subfloat[Planning with outliers]{%
  %   \resizebox{0.5\linewidth}{!}{
  %     \begin{tikzpicture}%
  %       \node at(0.0,0.0){\includegraphics[width=\linewidth,height=0.6\linewidth]{%
  %       ./images/fig1_path_w_outliers.png}};%
  %     \end{tikzpicture}}}%
  \caption{(a) \textbf{Chlorophyll-a sensing data}. The orange and red points are outliers~\cite{espinola2017statistical}. (b) \textbf{Ground-truth environmental model}. Green points are normal data points, and red points are outliers. Red and blue colors on the surface indicate high and low values, respectively. (c) \textbf{GPR without outliers} accurately predicts the environment and provides informative confidence bounds (i.e., the upper and lower black grids). (d) \textbf{GPR with outliers} leads to inaccurate ``flat'' prediction and uninformative uncertainty estimates, which further affects the performance of downstream informative planners.}%
  \label{fig:pull_figure}%
\end{figure}


==> figures/figure2.tex <==
\begin{figure}[tp]
  \centering
  \includegraphics[width=\linewidth]{images/figure2/system}
  % \includegraphics[width=\linewidth]{example-image}
  \caption{\textbf{System diagram}. (1) The Autonomous Surface Vehicle (ASV) collects depth measurements via the down-facing sonar. (2) An outlier detector keeps track of the outlier density across spatial locations (3) and passes the filtered data to the probabilistic model (4). The outlier density (5) and the predictive standard deviation (6) are fed to the multi-objective informative planner to guide the robot to collect the next batch of data.}%
  \label{fig:system}
\end{figure}


==> figures/figure3.tex <==
\begin{figure}[thbp]%
  \centering%
  \subfloat[]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth,height=0.8\linewidth]{images/figure3/outliers}};%
        % \includegraphics[width=\linewidth,height=0.8\linewidth,trim={50 20 60 20},clip]{example-image}};%
      \end{tikzpicture}}}%
  \subfloat[]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth,height=0.8\linewidth]{images/figure3/outliers_filtered}};%
        % \includegraphics[width=\linewidth,height=0.8\linewidth,trim={50 20 50 20},clip]{example-image}};%
      \end{tikzpicture}}}%
  \caption{(a) A matrix storing the outlier count at each spatial location. (b) A smoothed version of (a) using a Gaussian kernel. The smoothed outlier occurance matrix serves as one of the reward map in Pareto Monte Carlo tree search to revisiting sampling locations with outliers.}%
  \label{fig:outliers}%
\end{figure}


==> figures/figure4.tex <==
\begin{figure}[tp]%
  \centering%
  \subfloat{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \fbox{\includegraphics[width=\linewidth]{example-image}}};%
      \end{tikzpicture}}}%
  \subfloat{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \fbox{\includegraphics[width=\linewidth]{example-image}}};%
      \end{tikzpicture}}}\\%
  \subfloat{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \fbox{\includegraphics[width=\linewidth]{example-image}}};%
      \end{tikzpicture}}}%
  \subfloat{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \fbox{\includegraphics[width=\linewidth]{example-image}}};%
      \end{tikzpicture}}}%
  \caption{Illustrations of the searching results of PUCT and UCT. In the occupancy map of (a), black and white colors represent occupied space and free space, respectively. In a reward map, darker color indicates higher reward value. The goal is to search a trajectory that maximizes the cumulative reward. The green tree shows the searching process which outputs the best trajectory colored in red and best action shown in blue. The first reward map tells the PUCT to search towards the upper right while the second reward map encourages going up. The reward map of the UCT is the same as the first reward map in (a). The PUCT balances the two rewards and gives different trajectory at the end.}%
  \label{fig:puct}%
\end{figure}


==> figures/figure5.tex <==
\begin{figure*}[tp]%
  \centering%
  \subfloat[Ground truth\label{fig:gt}]{%
    \resizebox{0.33\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure5/env.png}};%
      \end{tikzpicture}}}%
  \subfloat[PUCT-COPOD\label{fig:puct_copod}]{%
    \resizebox{0.33\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure5/puct_copod.png}};%
      \end{tikzpicture}}}%
  \subfloat[UCT-COPOD\label{fig:uct_copod}]{%
    \resizebox{0.33\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure5/uct_copod.png}};%
      \end{tikzpicture}}}%
  \caption{Final predictive means of PUCT-COPOD and UCT-COPOD.}%
  \label{fig:prediction}%
\end{figure*}


==> figures/figure6.tex <==
\begin{figure}[thbp]%
  \centering%
  \subfloat[]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth,height=0.7\linewidth,trim={38 25 0 0},clip]{images/figure6/bezier}};%
      \end{tikzpicture}}}%
  \subfloat[]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth,height=0.7\linewidth]{images/figure6/uct_none_std}};%
      \end{tikzpicture}}}%
  \caption{(a) The Bezier curve to generate \emph{a priori} sampling path for collecting initial training data for the initial optimization of the GPR and computing data pre/post-processing statistics. (b) Final predictive standard deviation of UCT-NONE. }%
  \label{fig:bezier_std}%
\end{figure}


==> figures/figure7.tex <==
\begin{figure*}[tp]%
  \centering%
  \subfloat[$\rho=0.05$]{%
    \resizebox{0.43\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure7/rmses_005}};%
      \end{tikzpicture}%
    }%
  }%
  \subfloat[$\rho=0.10$]{%
    \resizebox{0.43\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure7/rmses_010}};%
      \end{tikzpicture}%
    }%
  }\\%
  \subfloat[$\rho=0.15$]{%
    \resizebox{0.43\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure7/rmses_015}};%
      \end{tikzpicture}%
    }%
  }%
  \subfloat[$\rho=0.10$]{%
    \resizebox{0.43\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure7/rmses_filter_all}};%
      \end{tikzpicture}}}%
  \caption{Root mean squared errors of the proposed PUCT-COPOD and other three baselines. UCT-BEST filters outliers with the ground-truth labels, so it serves as a best-case baseline; UCT-NONE, which is the worst case baseline, does not filter outliers at all. UCT-COPOD directly applies the outlier detector to the sensing data stream. Parameter $\rho$ controls the number of outliers: higher value indicates more outliers (MO) while lower value means less outliers (LO). In (a)-(c), the outlier detector only filters out the outliers in the newly acquired batch without changing the historical data. In (d), the outlier detector re-examine \emph{all} the historical data at each decision epoch. (a) Performance difference of all the methods is insignificant when the number of outliers is very small. (b) PUCT-COPOD and UCT-COPOD are both in between the best-case baseline and the worst-case baseline after collecting $1000$ samples while PUCT-COPOD performs better. At the early stage, UCT-COPOD is even worse than UCT-NONE because it filters out some informative samples. (c) When the number of outliers increases, UCT-COPOD loses advantage over UCT-NONE. The performance of PUCT-COPOD is also affected but its still better than UCT-COPOD and UCT-NONE. (d) Both PUCT-COPOD and UCT-COPOD are ineffective if the detector filters outliers in all historical data.}%
  \label{fig:rmse}%
\end{figure*}


==> figures/figure8.tex <==
\begin{figure}[thbp]%
  \centering%
  \subfloat[UCT-COPOD]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure8/uct_copod_samples}};%
      \end{tikzpicture}%
    }%
  }%
  \subfloat[PUCT-COPOD]{%
    \resizebox{0.5\linewidth}{!}{
      \begin{tikzpicture}%
        \node at(0.0,0.0){%
        \includegraphics[width=\linewidth]{images/figure8/puct_copod_samples}};%
      \end{tikzpicture}%
    }%
  }%
  \caption{(a) and (b) shows the absolute error maps and training samples after cleaning the outliers of UCT-COPOD and PUCT-COPOD, respectively. Many informative samples at the high-variability region are falsely filtered out in (a), leading to some high-error ``holes''. As a comparison, (b) shows that the proposed method can mitigate this effect to some extent.}%
  \label{fig:samples}%
\end{figure}

